A Quadratic Speedup in Finding Nash Equilibria of Quantum Zero-Sum Games

Recent developments in domains such as non-local games, quantum interactive proofs, and quantum generative adversarial networks have renewed interest in quantum game theory and, specifically, quantum zero-sum games. Central to classical game theory is the efficient algorithmic computation of Nash equilibria, which represent optimal strategies for both players. In 2008, Jain and Watrous proposed the first classical algorithm for computing equilibria in quantum zero-sum games using the Matrix Multiplicative Weight Updates (MMWU) method to achieve a convergence rate of $\mathcal{O}(d/\epsilon^2)$ iterations to $\epsilon$-Nash equilibria in the $4^d$-dimensional spectraplex. In this work, we propose a hierarchy of quantum optimization algorithms that generalize MMWU via an extra-gradient mechanism. Notably, within this proposed hierarchy, we introduce the Optimistic Matrix Multiplicative Weights Update (OMMWU) algorithm and establish its average-iterate convergence complexity as $\mathcal{O}(d/\epsilon)$ iterations to $\epsilon$-Nash equilibria. This quadratic speed-up relative to Jain and Watrous' original algorithm sets a new benchmark for computing $\epsilon$-Nash equilibria in quantum zero-sum games.

==> effort.tex <==
\subsection{Projections}

Mirror descent is an optimization algorithm that iteratively combines first-order oracle steps with a "mirror step", which is created by a projection-type mapping. The method originated from \cite{ny83}. The key element of this mirror step is a generalization of the Euclidean distance referred to as a "distance-generating" function:

\begin{definition}
\label{def:dgf}
A function $h:\mathcal{X}\to\mathbb{R}$ is called a \emph{distance-generating function} on $\mathcal{X}$ if:
\begin{enumerate}
\item
$h$ is continuous.
\item
$h$ is strongly convex, that is, there exists an $\alpha>0$ such that
\begin{equation}
\label{eq:StrongConvex}
h(\lambda x+(1-\lambda)x')
	\leq \lambda h(x)+(1-\lambda)h(x')-\frac{\alpha}{2}\lambda(1-\lambda)\norm{x-x'}^{2},
\end{equation}
for all $x,x'\in\mathcal{X}$ and all $\lambda\in[0,1]$.
\end{enumerate}
\end{definition}

The convex conjugate of a distance-generating function on $\mathcal{X}$ is given by
\begin{align}
h^{\ast}(y):=
	\max_{x\in\mathcal{X}} \{\langle{y,x}\rangle - h(x) \},
	\quad
	y\in\mathcal{Y},
\end{align}
and the associated \emph{mirror map} is defined as
\begin{equation}
\label{eq:Q}
Q(y):= \arg\max_{x\in\mathcal{X}} \{ \langle{y,x}\rangle - h(x) \}.
\end{equation}
Due to the strong convexity of $h$, $Q(y)$ is well-defined and single-valued for all $y\in\mathcal{Y}$. It performs a function similar to that of a projection mapping.

Our algorithm relies on variations of projected/mirror ascent methods. These iterative algorithms work by applying local improvements based on the gradient direction of the utility of the players and then projecting the current iterate onto a feasible set defined by problem constraints. This projection step ensures that the updated iterate remains within the feasible region. A generalization of this approach involves the use of a "mirror map," which characterizes the geometry of the feasible set and can impose additional structure or regularization on the optimization problem. In each iteration, mirror ascent computes a descent direction by taking a gradient step with respect to the mirror map, resulting in an update in the primal variables. This update is then adjusted based on the dual variables and the step size to ensure convergence. Mirror ascent offers flexibility in handling a wide range of optimization problems and allows for the incorporation of domain-specific knowledge into the optimization process.

This generalization plays a crucial role not only in multi-agent optimization but also in single-agent optimization. For instance, when maximizing a function $f$ on the spectraplex with subgradients bounded in the $\ell_{\infty}$-norm, mirror ascent with the von Neumann entropy achieves a convergence rate of approximately $\sqrt{\frac{\log n}{t}}$. On the other hand, regular subgradient descent only achieves a rate of approximately $\sqrt{\frac{ n}{t}}$ in this case \cite{BubeckConvexOptimizationBook}.

Throughout the paper, we will use three types of projection oracles, namely $(\orthproj_\mathcal{X} (\cdot), \bregproj^\regfunc_{\mathcal{X}}(\cdot), \mirproj^\regfunc_{\mathcal{X}}(\cdot,y))$, primarily to map potential candidate states onto a feasible set. We will later observe that the first projection corresponds to the second one under the Frobenius norm.

To refer to a projection onto the state space $\mathcal{X}$ generally, without specifying a specific form of projection, we will use the notation $\proj_\mathcal{X}(\cdot)$.


==> intro.tex <==
\begin{restatable}[1-MMP Rate]{theorem}{mainres}\label{thm:main-result}%
    1-MMP methods compute an $\epsilon$-Nash equilibrium in $\bigo({1}/{\epsilon})$ steps.
\end{restatable}
